A High-Throughput GPU Framework for Adaptive Lossless Compression of Floating-Point Data

The torrential influx of floating-point data from domains like IoT and HPC necessitates high-performance lossless compression to mitigate storage costs while preserving absolute data fidelity. Leveraging GPU parallelism for this task presents significant challenges, including bottlenecks in heterogeneous data movement, complexities in executing precision-preserving conversions, and performance degradation due to anomaly-induced sparsity. To address these challenges, this paper introduces a novel GPU-based framework for floating-point adaptive lossless compression. The proposed solution employs three key innovations: a lightweight asynchronous pipeline that effectively hides I/O latency during CPU-GPU data transfer; a fast and theoretically guaranteed float-to-integer conversion method that eliminates errors inherent in floating-point arithmetic; and an adaptive sparse bit-plane encoding strategy that mitigates the sparsity caused by outliers. Extensive experiments on 12 diverse datasets demonstrate that the proposed framework significantly outperforms state-of-the-art competitors, achieving an average compression ratio of 0.299 (a 9.1% relative improvement over the best competitor), an average compression throughput of 10.82 GB/s (2.4x higher), and an average decompression throughput of 12.32 GB/s (2.4x higher).

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}
%讨论32位的方案
%对于32位数据，
\subsection{Adapting Falcon for Single-Precision Data}\label{sec:32bit}

The adaptation of the Falcon framework to support single-precision floating-point numbers is straightforward, and importantly, our core theoretical foundations remain fully applicable. The key difference lies in the adjustment of the safe operating bounds for the conversion due to the reduced bit-depth of the single-precision format.
The IEEE 754 single-precision format provides a 24-bit mantissa (23 bits stored plus one hidden bit), compared to the 53-bit mantissa in double-precision. This directly impacts the maximum integer value that can be represented without precision loss. Consequently, the conditions in our theorems must be updated:

Theorem~\ref{the:round} (Conversion Correctness) and \textit{Theorem~\ref{the:recoverable} (Conversion Recoverability)} are still valid. However, the maximum decimal significand ($\hat{\beta}$) and decimal place ($\alpha$) that can be guaranteed for lossless conversion are reduced. Our analysis shows that for single-precision, the safe bounds are approximately $\hat{\beta} \le 6$ (down from 15) and $\alpha \le 10$ (down from 22). These new bounds ensure that both the scaled integer ($\text{round}(v \otimes 10^\alpha)$) and the scaling factor ($10^\alpha$) can be perfectly represented within the 24-bit mantissa.
The decimal place calculation logic (Theorem~\ref{thm:conversionErrorBound} and Algorithm~\ref{alg:DPAndDSCalculation}) remains entirely correct. The algorithm's loop for finding the correct $\alpha$ simply uses these new, stricter bounds ($\alpha \le 10$ and $\hat{\beta} \le 6$) as its termination condition.

For any 32-bit floating-point number that exceeds these limits, Falcon's adaptive mechanism automatically and correctly defaults to the alternative bitwise conversion method (Case 2), guaranteeing losslessness across all possible data ranges.
%讨论FOR的方案
%
\subsection{Integration of Frame-of-Reference Methods}

While our current implementation uses a delta encoding to reduce the magnitude of converted integers, incorporating a Frame-of-Reference (FOR) approach presents another viable strategy. In a FOR scheme, a block of data is encoded as smaller offsets from a single reference value (often the minimum value within the block). This can be particularly effective for data chunks that exhibit high local correlation.

FOR methods are highly compatible with the Falcon architecture. Specifically, after the initial float-to-integer conversion, a FOR encoding step could directly replace the current delta encoding ($z_i = \text{Zigzag}(g_i - g_{i-1})$). A seemingly optimal approach would be a hybrid model where the system dynamically selects between delta encoding and FOR for each data chunk based on which method yields better compression. However, this dynamic selection introduces a critical performance bottleneck on GPUs due to \emph{warp divergence}. If different threads within the same warp process data chunks with different statistical properties, they would diverge into separate execution paths (one for FOR, one for delta). This forces the GPU to serialize their execution, negating the benefits of parallel processing and severely degrading overall throughput.

Therefore, to ensure consistently high throughput and architectural simplicity, we opted for the more \textbf{robust} delta encoding algorithm. It avoids the risk of a suboptimal reference value selection in FOR, which can, in some cases, lead to larger encoded values and a degraded compression ratio. The delta encoding method is computationally lightweight and demonstrates strong, reliable performance across diverse datasets, making it a more predictable and generally effective choice for a high-throughput parallel framework.

==> gpu.tex <==
%  \section{GPU-Based Acceleration}\label{sec:gpu}
% %为了提升浮点数据压缩算法在大规模场景下的运行效率，我们设计了一套基于 GPU 的并行加速方案。该方案从显存管理、并发调度和核函数优化三个方面出发，旨在充分利用 GPU 的计算能力与内存带宽，减少内存开销并提高压缩吞吐量。
% To enhance the execution efficiency of floating-point data compression algorithms in large-scale scenarios, we propose a CPU-GPU heterogeneous scheduling framework. This scheme integrates GPU memory pool management and a self-adaptive multi-stream concurrency mechanism, aiming to overlap data transfer latency with computation, reduce memory overhead, and maximize compression throughput.
% \subsection{Memory Pool Management Mechanism}
% %在 GPU 上执行大规模数据压缩任务时，频繁的显存分配（cudaMalloc）与释放（cudaFree）会显著增加运行开销，尤其在多流并发的情况下，显存资源的管理变得更加复杂。为了提高显存的利用效率，我们设计了一个显存池管理机制，通过双显存池管理原始数据和压缩数据的显存资源。
% When executing large-scale data compression tasks on GPUs, frequent memory allocation (\texttt{cudaMalloc}) and deallocation (\texttt{cudaFree}) significantly increase the runtime overhead, especially when using multiple concurrent streams. To improve memory utilization, we have designed a memory pool management mechanism that uses two separate memory pools to manage the memory resources for raw data and compressed data.
% %我们通过两个显存池来分别管理不同的数据：原始数据显存池（Origdata Pool）：用于存储待压缩的原始浮点数据。每个 CUDA 流从这个池中申请内存块进行数据传输。并在压缩计算后立即释放。压缩数据显存池（Cmpdata Pool）：用于存储压缩后的中间结果，直到压缩结果从 GPU 拷贝回主机。压缩任务完成后，压缩结果被异步回传主机，之后显存池中的内存块被释放。
% We use two memory pools to manage different types of data:
% \begin{itemize}
%     \item \textbf{Raw Data Memory Pool (Origdata Pool)}: This pool stores the raw floating-point data to be compressed. Each CUDA stream allocates memory blocks from this pool for data transfer and releases them immediately after compression computation.
%     \item \textbf{Compressed Data Memory Pool (Cmpdata Pool)}: This pool stores the intermediate results of the compression process until the compressed results are copied back to the host from the GPU. After the compression task is completed, the compressed results are asynchronously transferred back to the host, and the memory blocks in the pool are then released.
% \end{itemize}

% %在程序初始化阶段，通过 cudaMalloc 为整个显存池分配一块连续的显存区域，随后将显存区域按每个压缩任务所需的内存大小（chunkSize）划分成多个固定大小的内存块。每个 CUDA 流在执行时，从显存池中动态申请内存块，并在任务完成后将内存块归还给显存池。
% During the system initialization phase, based on the available free GPU memory, two contiguous memory regions are allocated for the memory pools using \texttt{cudaMalloc}. These regions are divided into fixed-size memory chunks according to the block size required for each compression task (\texttt{chunkSize}). 


% \subsection{Self-adaptive Multi-stream Concurrency Mechanism}

% %为了进一步提升压缩系统的并行能力和吞吐性能，我们在 GPU 执行框架中引入了 多 CUDA 流（multi-stream）并发调度机制。该机制允许多个任务同时在 GPU 上执行，并实现数据传输（memory copy）与压缩计算（kernel execution）的异步重叠，从而最大程度地发挥 GPU 的计算能力和内存带宽。
% To further enhance the parallelism and throughput performance of the compression system, we introduced a \textbf{multi-stream concurrent scheduling mechanism} in the GPU execution framework. This mechanism allows multiple tasks to be executed simultaneously on the GPU and enables asynchronous overlap between data transfer (memory copy) and compression computation (kernel execution), thus maximizing the GPU's computational power and memory bandwidth.

% % 在本系统中，每个 CUDA 流被视为一个独立的任务通道，负责执行一次压缩流程，包括数据拷贝、压缩计算以及结果回传。为了优化数据上传的速度，我们使用了 页锁内存（Pinned Memory），使得数据能够通过直接内存访问（DMA）进行快速传输，避免了传统内存传输中操作系统的虚拟内存管理所带来的延迟，从而加速了数据从主机到设备的传输。
% In our system, each CUDA stream is treated as an independent task channel responsible for executing a complete compression process, including data copy, compression computation, and result transfer. To optimize the data upload speed, we use \textbf{pinned memory} for the raw data pool. Pinned memory is locked in physical memory, avoiding the overhead caused by virtual memory management in typical pageable memory. By utilizing pinned memory, data can be transferred to the GPU using \textbf{direct memory access (DMA)}, significantly speeding up data transfers from the host to the device and reducing the data transfer delay. This improvement allows more time for the subsequent computation phase.


% %改这里

% % 整个流程中，多个 CUDA 流彼此独立、相互协作，构成一种流水线式并行调度架构。当某一流处于数据传输阶段时，另一流可能正处于计算阶段或结果传输阶段，实现了数据搬运与计算的重叠，大幅减少 GPU 空闲时间。                                      
% Throughout the process, multiple CUDA streams work independently and collaboratively, forming a pipeline-like parallel scheduling architecture. When one stream is in the data transfer phase, another stream may be in the computation or result transfer phase. In this way, data movement and computation tasks can effectively overlap, significantly reducing GPU idle time and increasing overall throughput.

% % 此外，结合显存池机制，每个 CUDA 流可以从统一的显存资源池中动态申请和释放内存块，实现资源的复用与高效调度，避免了传统方式中“每个流绑定固定显存块”带来的浪费与限制。
% Additionally, combined with the memory pool mechanism, each CUDA stream can dynamically allocate and release memory blocks from a unified memory pool, ensuring resource reuse and efficient scheduling. This avoids the resource wastage and limitations caused by traditional methods where each stream is bound to a fixed memory block. By dynamically allocating memory and utilizing pinned memory, we ensure efficient parallel execution of data transfer and computation tasks, which further enhances system performance.
% %合理的流数量对于压缩任务的并行执行至关重要。若流数设置过少，将导致 GPU 中部分执行单元或传输通道处于空闲状态；而流数设置过多，则可能引发调度开销、上下文切换频繁等问题。我们基于压缩任务中各阶段耗时的分布规律，结合延迟隐藏模型，推导出合理的最小流数量估算公式：
% The number of streams is crucial for parallel execution of compression tasks. If too few streams are used, some GPU execution units or transmission channels may remain idle, wasting computational resources. On the other hand, if too many streams are used, scheduling overhead and frequent context switching may arise. Therefore, we need to select the optimal number of streams based on the time distribution of each stage. Based on the latency hiding model and the time distribution of each phase in the compression task, we derive a reasonable estimation formula for the minimum number of streams required to maximize the overlap between data transfer and computation:

% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{figures/stream.pdf}
%   \caption{Multi-Stream Concurrent Scheduling Architecture}
%   \label{fig:stream}
% \end{figure}


\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/4stage.pdf}
  \caption{A Comparison of Pipeline Models for Variable-Sized Outputs.}
  \label{fig:4stage}
\end{figure}

\section{GPU-Based Acceleration}\label{sec:gpu}

\subsection{The Challenge of Deep Pipelining on GPUs}
% GPU的大规模并行性提供了巨大的原始计算能力，但实现高应用吞吐量的瓶颈通常不在于计算本身，而在于如何持续地为处理核心供给数据。这就要求我们必须采用一个流水线执行模型（pipelined execution model），在其中，CPU-GPU之间巨大的数据传输延迟，可以通过与核函数计算的重叠而被隐藏起来。虽然多流流水线是实现这种重叠的标准架构，但它在数据压缩场景下面临一个根本性的困境：每个数据块的输出大小是可变的，且事前未知。这种可变性打破了简单的三阶段（HtoD -> Kernel -> D2H）模型，因为主机无法在不大量浪费内存或引入阻塞流水线的同步步骤的情况下，为D2H阶段预先分配一个大小精确的缓冲区。
 The massive parallelism of a GPU offers tremendous raw computational power, but achieving high application throughput is often limited not by computation, but by keeping the processing cores fed with data. This necessitates a pipelined execution model, where the substantial latency of CPU-GPU data transfers is hidden by overlapping it with kernel computation. While a multi-stream pipeline is the standard architecture for achieving such overlap, it confronts a fundamental dilemma in data compression: the output size of each data chunk is variable and unknown beforehand. This variability breaks the simple three-stage (H2D -> Kernel -> D2H) model, as the host cannot pre-allocate a precisely-sized buffer for the D2H stage without either wasting significant memory or introducing a pipeline-stalling synchronization step. 
 
 %因此，为了构建一个真正有效的流水线，我们的框架基于一个更先进的调度架构。它采用了一个将元数据与载荷解耦的多阶段流水线模型，并由一个非阻塞的、事件驱动的调度器来编排，从而同时实现了最大吞吐量和高内存效率。
 Therefore, to build a truly effective pipeline, our framework is based on a more advanced scheduling architecture. It employs a multi-stage pipeline model that decouples the transfer of metadata (compressed size) from its corresponding data payload (compressed data) and is orchestrated by a non-blocking, event-driven scheduler, enabling both maximum throughput and high memory efficiency.

\subsection{The Four-Stage Asynchronous Pipeline Model}
%一个标准的GPU任务流水线方法包含三个阶段：主机到设备传输（HtoD）、核函数执行、以及设备到主机传输（D2H）。然而，在处理像数据压缩这样输出大小可变的任务时，这个模型会遇到一个根本性的困境。主机必须在启动D2H拷贝之前，分配一个缓冲区来接收压缩数据，这导致了两种次优的策略，如图7所示。
A standard approach to pipelining GPU tasks involves a three-stage model: Host-to-Device transfer (H2D), Kernel execution, and Device-to-Host transfer (D2H). This model, however, encounters a fundamental dilemma when processing tasks with variable-sized outputs, such as data compression. The host must allocate a buffer to receive the compressed data before initiating the D2H copy, leading to two suboptimal strategies, as illustrated in Figure~\ref{fig:4stage}.

% 第一种策略，如图7(a)所示，是过度分配（Over-provisioning）。主机为每一次D2H传输都分配一个最坏情况下的缓冲区，其大小通常等于原始未压缩块的大小。尽管这能让流水线无停顿地运行，但它会导致主机端严重的内存浪费和碎片化，尤其是在压缩率很高的情况下，需要进一步对碎片进行处理。
The first strategy, shown in Figure~\ref{fig:4stage}(a), is Static Buffer Allocation. The host allocates a worst-case buffer for each D2H transfer, often equal to the size of the original uncompressed chunk. While this allows the pipeline to run without stalls, it leads to significant memory waste and fragmentation on the host, especially when compression ratios are high, requiring further fragmentation processing.

%另一种策略，如图7(b)所示，依赖于同步元数据获取（Synchronous Metadata Fetch）。在这个模型中，流水线在核函数执行后被迫停顿（stall）。一个阻塞式的D2H操作被执行，用以首先取回压缩后的大小。这引入了一个巨大的流水线停顿（或同步气泡），它使原本并行的工作流串行化，并急剧降低了整体吞吐量。
The alternative strategy, shown in Figure~\ref{fig:4stage}(b), relies on a Synchronous Metadata Fetch. In this model, the pipeline is forced to Synchronous after kernel execution. A blocking D2H operation is performed to retrieve the compressed size first. This introduces a severe synchronization bubble, which serializes the otherwise parallel workflow and drastically reduces overall throughput.

%为了系统性地将计算与数据传输进行重叠，我们将单个数据块的端到端压缩过程分解为一个四阶段异步流水线。该模型如图6所示，构成了我们调度框架的骨架。每个阶段都被设计为在CUDA流上以异步操作的方式启动。
To resolve this dilemma, we propose our novel four-stage asynchronous pipeline model, shown in Figure~\ref{fig:4stage}(c). Our key insight is to decouple the transfer of metadata (the compressed size) from the transfer of the payload (the compressed data). This transforms the problematic single D2H stage into two distinct, lightweight, and asynchronous stages:

% 阶段1：主机到设备（H2D）数据传输： 原始数据块从主机的内存异步地拷贝到GPU的全局内存。为最大化传输速度，主机端的缓冲区被分配为页锁定（Pinned）内存，以启用直接内存访问（DMA）。
% 阶段2：核函数执行： 在GPU上启动FALCON-g压缩核函数。该核函数执行第4章详述的完整自适应压缩策略，将GPU内存中的原始数据块转换为压缩表示。
% 阶段3：元数据设备到主机（D2H）传输： 核函数完成后，一小块固定大小的元数据——即压缩块的大小（CmpSize）——被异步地拷贝回主机。
% 阶段4：载荷数据设备到主机（D2H）传输： 一旦主机接收到CmpSize，它就可以在其内存中分配一个精确大小的缓冲区。随后，它启动最后的异步拷贝，将大小可变的压缩载荷从GPU传输到这个新分配的缓冲区中。
\textbf{Stage 1: Host-to-Device (H2D) Data Transfer:} The raw data chunk is asynchronously copied to the GPU. A critical design choice is the use of \textbf{page-locked memory} for the host-side buffers. This provides two essential benefits: 1) it enables faster Direct Memory Access (DMA) transfers, and 2) it ensures a truly non-blocking host operation by eliminating the hidden synchronization that occurs with standard pageable memory.

\textbf{Stage 2: Kernel Execution:} The FALCON-g compression kernel is launched on the GPU. This kernel executes the entire adaptive compression strategy detailed in Section~\ref{sec:method}, transforming the raw data chunk into a compressed representation within the GPU's memory.


\textbf{Stage 3: Metadata Device-to-Host (M-D2H) Transfer:} Upon kernel completion, a small, fixed-size piece of metadata—the size of the compressed chunk (\texttt{CmpSize})—is asynchronously copied back to the host.


\textbf{Stage 4: Payload Device-to-Host (P-D2H) Transfer:} Once the host receives the \texttt{CmpSize}, it can allocate a precisely sized buffer in its memory. It then initiates the final asynchronous copy of the variable-sized compressed payload from the GPU to this newly allocated buffer.

%这种两阶段D2H策略优雅地解决了这个问题。元数据传输因其体积小且固定而速度飞快。在其完成后，主机可以为载荷数据进行一次“即时”且大小精确的内存分配。至关重要的是，这整个依赖关系都通过CUDA事件（详见5.3节）进行异步管理，维持了流水线的流畅性，而没有引入任何阻塞式同步。这使我们能够同时实现主机端的高内存效率和流水线的最大吞吐量。
This two-phase D2H strategy elegantly solves the problem. The metadata transfer is fast due to its small, fixed size. Upon its completion, the host can perform a just-in-time, precisely sized memory allocation for the payload. Crucially, this entire dependency is managed asynchronously using CUDA Events (as detailed in Section 5.3), preserving the fluidity of the pipeline without introducing any blocking synchronization. This allows us to achieve both high memory efficiency on the host and maximum pipeline throughput.

\subsection{The Event-Driven State Scheduler}
% 为了管理我们四阶段流水线的复杂依赖关系，我们设计了一个轻量级且可扩展的事件驱动调度框架。该框架在主机上运行，并编排整个工作流程，确保操作之间的最大化重叠，而无需借助昂贵的阻塞式同步。
To manage the complex dependencies of our four-stage pipeline, we designed a lightweight and scalable Event-Driven Scheduling Framework. This framework operates on the host and orchestrates the entire workflow, ensuring maximum overlap between operations without resorting to expensive, blocking synchronization.

\subsubsection{State and Dependency Management}The core of our framework is a simple \textbf{state machine} that tracks the progress of each data chunk. For each of the $N$ concurrent CUDA streams, we maintain a state variable, \texttt{stage[s]}, which can be in one of the following three states: \texttt{IDLE}, \texttt{SIZE\_PENDING}, or \texttt{DATA\_PENDING}.

The transition between these states is governed not by blocking calls, but by \textbf{CUDA Events}, which are lightweight synchronization primitives that act as non-blocking signals from the GPU. Two events, \texttt{evSize[s]} and \texttt{evData[s]}, are associated with each stream. The \texttt{evSize[s]} event is recorded after the M-D2H stage, and \texttt{evData[s]} is recorded after the P-D2H stage. This allows the host scheduler to precisely track the completion of asynchronous GPU operations without stalling.
% 这些状态之间的转换并非由阻塞调用驱动，而是由**CUDA事件（CUDA Events）**驱动。正如我们的实现所示，每个流s都关联了两个事件 evSize[s] 和 evData[s]。evSize[s] 事件在CmpSize元数据拷贝（阶段3）入队后立即被记录，而 evData[s] 在最终的载荷拷贝（阶段4）后被记录。这些事件作为非阻塞信号，允许调度器在不造成停顿的情况下查询一个操作的状态。

\subsubsection{The Non-Blocking Scheduling Loop}
%5.3.2 非阻塞调度循环
% 调度器的逻辑被实现为主机上的一个连续循环，它迭代遍历所有NUM_STREAMS。这个基于轮询的非阻塞循环（如我们代码中的while循环所示）构成了我们流水线的引擎。在循环内部，一个switch语句检查每个流的当前stage并采取相应行动：
The engine of our scheduling framework is a central dispatch loop on the host, which implements a state-driven, non-blocking polling model. This loop systematically orchestrates the progression of each data chunk through the pipeline. It continuously traverses the array of NUM\_STREAMS, querying the state of each and taking action accordingly. 

1. \textit{Pipeline Initiation (\texttt{IDLE} state).}
When the dispatcher encounters an \texttt{IDLE} stream, it launches the initial sequence of operations for a new data chunk onto this stream: Host-to-Device  transfer (Stage~1), Kernel Execution (Stage~2), and Metadata Device-to-Host Transfer (Stage~3). It then records the \texttt{evSize[s]} event, updates the stream's state to \texttt{SIZE\_PENDING}, and immediately proceeds to the next stream.

2. \textit{Dependency Resolution (\texttt{SIZE\_PENDING} state).}
For a stream in this state, the dispatcher performs a non-blocking query on the \texttt{evSize[s]} event. If the event has completed, it signals that the dependency for Stage~4 has been met. The dispatcher then launches the final Payload D2H Transfer (Stage~4), records the \texttt{evData[s]} event, and transitions the state to \texttt{DATA\_PENDING}. If the event is not ready, the dispatcher simply continues to the next stream, avoiding any stalls.

3. \textit{Pipeline Completion and Resource Recycling (\texttt{DATA\_PENDING} state).}
In this final state, the dispatcher polls the \texttt{evData[s]} event. Its completion signifies that a data chunk has been fully processed. The dispatcher then transitions the stream's state back to \texttt{IDLE}. This action effectively recycles the stream, making it immediately available for a new data chunk and ensuring the pipeline remains deeply and continuously filled.

While this non-blocking model maximizes throughput under normal conditions, it is susceptible to a potential livelock scenario. If all active streams are simultaneously waiting for GPU events that are unexpectedly delayed (e.g., due to heavy system load or resource contention), the host loop could poll indefinitely without making forward progress.


To ensure the framework's robustness, we integrate a livelock prevention mechanism. At the end of each full traversal of the stream array, the scheduler checks if any forward progress was made (i.e., if any stream changed its state). If an entire polling cycle completes with no progress, the scheduler temporarily breaks the non-blocking pattern. It performs a targeted, blocking synchronization by calling cudaStreamSynchronize() on the oldest "in-flight" stream.


This strategic, conditional synchronization is a critical safeguard that guarantees forward progress. By forcing the system to complete at least one pending GPU operation, it ensures that the pipeline will not get stuck in an indefinite waiting loop. This prevention mechanism makes our entire asynchronous framework more robust and resilient to unpredictable scheduling behaviors, without sacrificing performance during normal, high-throughput execution.



% \begin{enumerate}
%     \item \textbf{If a stream is \texttt{IDLE}}, and there is more data to process, the scheduler initiates the first part of the pipeline. It launche   s the \textit{HtoD Data Transfer} (Stage~1), the \textit{Kernel Execution} (Stage~2), and the \textit{Metadata D2H Transfer} (Stage~3), all on the same stream $s$. Crucially, it then records the \texttt{evSize[s]} event and transitions the stream's state to \texttt{SIZE\_PENDING}. The scheduler then immediately moves to the next stream without waiting.

%     \item \textbf{If a stream is \texttt{SIZE\_PENDING}}, the scheduler performs a non-blocking query on its \texttt{evSize[s]} event using \texttt{cudaEventQuery}.
%     \begin{itemize}
%         \item If the event has not completed (\texttt{cudaErrorNotReady}), the scheduler does nothing and proceeds to the next stream, avoiding any stalls.
%         \item If the event has completed (\texttt{cudaSuccess}), it signifies that \texttt{CmpSize} is available on the host. The scheduler then uses this size to launch the \textit{Payload D2H Transfer} (Stage~4), records the \texttt{evData[s]} event, and transitions the state to \texttt{DATA\_PENDING}.
%     \end{itemize}

%     \item \textbf{If a stream is \texttt{DATA\_PENDING}}, a similar non-blocking query is performed on \texttt{evData[s]}. Upon its completion, the scheduler knows the chunk has been fully processed. It transitions the stream's state back to \texttt{IDLE}, making it available for a new data chunk, and the cy cle repeats.
% \end{enumerate}

% \subsubsection{Scalability and Performance Implications}

% This event-driven, polling-based architecture is the key to our framework's performance and scalability.

% \begin{itemize}
%     \item \textbf{High Responsiveness:} The non-blocking nature of \texttt{cudaEventQuery} ensures the host scheduler is never stalled. It can rapidly cycle through all active streams, launching new work as soon as dependencies are met. This makes the system highly responsive and maximizes the overlap of operations.

%     \item \textbf{Low Overhead:} The state management is extremely lightweight, consisting of only a few variables per stream. This allows the framework to scale to a large number of concurrent streams with negligible scheduling overhead.

%     \item \textbf{Resource Maximization:} By keeping the pipeline constantly fed and progressing, the scheduler ensures that the GPU's computational cores and data transfer engines are kept busy, leading to maximal system throughput.
% \end{itemize}

\subsection{Asymmetric Pipeline Design: A Simplified Three-Stage Model for Decompression}

While the compression pipeline requires a sophisticated four-stage model to handle variable-sized outputs, the decompression process is inherently simpler and allows for a more streamlined approach. This leads to an \textit{asymmetric pipeline design}, where decompression employs a traditional and highly efficient three-stage (H2D $\rightarrow$ Kernel $\rightarrow$ D2H) pipeline, as illustrated in Figure~\ref{fig:4stage}(a) (with roles reversed).

The key difference lies in the predictability of output sizes. During decompression, the size and location of each compressed data chunk are known beforehand, typically read from a metadata header or an offset array. Similarly, the size of the original, uncompressed data chunk is also known or can be easily stored. This critical information allows the host to \textbf{pre-allocate precisely-sized buffers} for the decompressed data before launching the decompression kernel.

With the output buffer size being fixed and known, the fundamental dilemma of variable-sized outputs vanishes. Consequently, the decompression workflow simplifies to:

\begin{enumerate}
    \item \textbf{Stage 1: Host-to-Device (H2D) Transfer}. The compressed data chunks are asynchronously copied from host memory to the GPU.
    
    \item \textbf{Stage 2: Decompression Kernel}. The FALCON-g decompression kernel is launched. It reads the compressed chunks and writes the reconstructed data directly into a pre-allocated output buffer on the GPU.
    
    \item \textbf{Stage 3: Device-to-Host (D2H) Transfer}. The final, reconstructed data is asynchronously copied back from the GPU to a precisely-sized buffer on the host.
\end{enumerate}

This simplified three-stage model for decompression avoids the complexity of the decoupled metadata transfer (M-D2H) and payload transfer (P-D2H) stages required for compression. It eliminates the need for an event-driven state scheduler to manage complex dependencies, resulting in lower overhead and maximizing throughput for the decompression workload. This asymmetric design ensures that both compression and decompression are optimized according to their unique characteristics, delivering the best possible end-to-end performance.
